Comparing seven methods for state-of-health time series prediction for the lithium-ion battery packs of forklifts

A key aspect for the forklifts is the state-of-health (SoH) assessment to ensure the safety and the reliability of uninterrupted power source. Forecasting the battery SoH well is imperative to enable preventive maintenance and hence to reduce the costs. This paper demonstrates the capabilities of gradient boosting regression for predicting the SoH timeseries under circumstances when there is little prior information available about the batteries. We compared the gradient boosting method with light gradient boosting, extra trees, extreme gradient boosting, random forests, long short-term memory networks and with combined convolutional neural network and long short-term memory networks methods. We used multiple predictors and lagged target signal decomposition results as additional predictors and compared the yielded prediction results with different sets of predictors for each method. For this work, we are in possession of a unique data set of 45 lithium-ion battery packs with large variation in the data. The best model that we derived was validated by a novel walk-forward algorithm that also calculates point-wise confidence intervals for the predictions; we yielded reasonable predictions and confidence intervals for the predictions. Furthermore, we verified this model against five other lithium-ion battery packs; the best model generalised to greater extent to this set of battery packs. The results about the final model suggest that we were able to enhance the results in respect to previously developed models. Moreover, we further validated the model for extracting cycle counts presented in our previous work with data from new forklifts; their battery packs completed around 3000 cycles in a 10-year service period, which corresponds to the cycle life for commercial Nickel-Cobalt-Manganese (NMC) cells.

==> junk.tex <==
@article{aro18mec,
	author={S. Arora et al.},
	year={2016},
	title={Review of mechanical design and strategic placement technique of a robust battery pack for electric vehicles},
	journal={Renewable \& sustainable energy reviews},
	volume={60},
	pages={1319-1331},
	isbn={1364-0321},
	doi={10.1016/j.rser.2016.03.013}
}
@misc{har17hyb},
	author={S. C. Harris},
	year={2017},
	month={28 February},
	title={Hybrid vehicle with modular battery system},
	number={U.S. patent 9,579,961}
}
@article{aro18app,
	author={S. Arora et al.},
	year={2018},
	title={Application of Robust Design Methodology to Battery Packs for Electric Vehicles: Identification of Critical Technical Requirements for Modular Architecture},
	journal={Batteries},
	volume={4},
	number={3},
	pages={30},
	isbn={2313-0105},
	doi={10.3390/batteries4030030}
}
@article{kra05com,
	author={P. Krause et al.},
	year={2005},
	title={Comparison of different efficiency criteria for hydrological model assessment},
	journal={Advances in Geosciences},
	volume={5},
	pages={89-97},
	isbn={1680-7340},
	doi={10.5194/adgeo-5-89-2005}
}
@misc{ano20pyt,
	author={anonymous},
	year={2020},
	title={Python sckikit.learn library function sklearn.model\_selection.TimeSeriesSplit},
	volume={2020},
	number={11.August},
	url={https://scikit-learn.org/stable/modules/generated/sklearn.model_selection.TimeSeriesSplit.html}
}
@article{bre96bag,
	author={L. Breiman},
	year={1996},
	title={Bagging predictors},
	journal={Machine Learning},
	volume={24},
	number={2},
	pages={123-140},
	isbn={0885-6125},
	doi={10.1007/BF00058655}
}
@book{has01ele,
	author={T. Hastie, J. Friedman and R. Tibshirani},
	year={2001},
	title={The Elements of Statistical Learning},
	publisher={Springer New York},
	pages={xvi-%20533},
	isbn={0-387-95284-5}
}
@misc{nau14ARI,
	author = 	 {F. Nau},
	year = 	 {2014},
	title = 	 {ARIMA models},
	journal = 	 {Lecture notes},
	url = 	 {http://people.duke.edu/~rnau/Slides_on_ARIMA_models--Robert_Nau.pdf}
}
@book{hyn19for,
	author={R. Hyndman and G. Athanasopoulos},
	year={2019},
	title={Forecasting Principles and Practise},
	publisher={OTexts},
	address={Melbourne, Australia},
	edition={3},
	pages={Chapter 8},
	isbn={978-0-9875071-0-5.},
	url={https://otexts.com/fpp3/}
}
@inproceedings{che16XGB,
	author={T. Chen and C. Guestrin},
	year={2016},
	month={August 13-17, 2016},
	title={XGBohynost: A Scalable Tree Boosting System},
	publisher={ACM},
	address={San Francisco, CA, USA},
	pages={785–794},
	doi={http://dx.doi.org/10.1145/2939672.2939785}
}
@book{box08tim,
	author={G. Box, G. M. Jenkins and G. C. Reinsel},
	year={2008},
	title={Time Series Analysis: Forecasting and Control, Fourth Edition},
	publisher={Wiley},
	volume={10},
	pages={1-746},
	isbn={0-470-27284-8}
}
@article{aro18ano,
	author={S. Arora et al.},
	year={2018},
	title={A novel thermal management system for improving discharge/charge performance of Li-ion battery packs under abuse},
	journal={J–ournal of Power Sources},
	volume={378},
	pages={759-775},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2017.12.030}
}
@article{aro18sel,
	author={S. Arora},
	year={2018},
	title={Selection of thermal management system for modular battery packs of electric vehicles: A review of existing and emerging technologies},
	journal={Journal of Power Sources},
	volume={400},
	pages={621-640},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2018.08.020}
}
@article{fle16int,
	author={M. Fleischhammer et al.},
	year={2015},
	title={Interaction of cyclic ageing at high-rate and low temperatures and safety in lithium-ion batteries},
	journal={Journal of Power Sources},
	volume={274},
	pages={432-439},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2014.08.135}
}
@article{zha20per,
	author={Y. Zhang et al.},
	year={2020},
	title={Performance assessment of retired EV battery modules for echelon use},
	journal={Energy (Oxford)},
	volume={193},
	pages={1-435},
	isbn={0360-5442},
	doi={10.1016/j.energy.2019.116555}
}
@article{mak18sta,
	author={S. Makridakis et al.},
	year={2018},
	title={Statistical and Machine Learning forecasting methods: Concerns and ways forward},
	journal={PLoS ONE},
	volume={13},
	number={3},
	pages={e0194889},
	isbn={1932-6203},
	doi={10.1371/journal.pone.0194889}
}
@article{mak18M4,
	author={S. Makridakis et al.},
	year={2018},
	title={The M4 Competition: Results, findings, conclusion and way forward},
	journal={International Journal of Forecasting},
	volume={34},
	number={4},
	pages={802-808},
	isbn={0169-2070},
	doi={10.1016/j.ijforecast.2018.06.001}
}
@article{mak00M3,
	author={S. Makridakis et al.},
	year={2000},
	title={The M3-Competition: Results, conclusions and implications},
	journal={International Journal of Forecasting},
	volume={16},
	number={4},
	pages={451-476},
	isbn={0169-2070},
	doi={10.1016/S0169-2070(00)00057-1}
}
@book{rus13AI,
	author={Stuart Russell and Peter Norvig},
	year={2013},
	title={Artificial Intelligence: Pearson New International Edition},
	publisher={Pearson},
	isbn={1-292-02420-8}
}
@article{bir17deg,
	author={C. Birkl et al.},
	year={2017},
	title={Degradation diagnostics for lithium ion cells},
	journal={Journal of Power Sources},
	volume={341},
	number={C},
	pages={373-386},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2016.12.011}
}
@article{far15cri,
	author={A. Farmann et al.},
	year={2015},
	title={Critical review of on-board capacity estimation techniques for lithium-ion batteries in electric and hybrid electric vehicles},
	journal={Journal of Power Sources},
	volume={281},
	pages={114-130},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2015.01.129}
}
@article{att20clo,
	author={P. Attia},
	year={2020},
	title={Closed-loop optimization of fast-charging protocols for batteries with machine learning.},
	journal={Nature},
	volume={578},
	number={7795},
	pages={397-402},
	isbn={0028-0836},
	doi={10.1038/s41586-020-1994-5}
}
@article{sev19dat,
	author={K. Severson et al.},
	year={2019},
	title={Data-driven prediction of battery cycle life before capacity degradation},
	journal={Nature Energy},
	volume={4},
	number={5},
	pages={383-391},
	isbn={2058-7546},
	doi={10.1038/s41560-019-0356-8}
}
@article{lei20mul,
	author={C. Lei et al.},
	year={2020},
	title={Multi-objective Optimization of Data-driven Model for Lithium-ion Battery SOH estimation with Short-term Feature},
	journal={IEEE Transactions on Power Electronics},
	pages={1},
	isbn={0885-8993},
	doi={10.1109/TPEL.2020.2987383}
}
@article{nuh13hea,
	author={A. Nuhic et al.},
	year={2013},
	title={Health diagnosis and remaining useful life prognostics of lithium-ion batteries using data-driven methods},
	journal={Journal of Power Sources},
	volume={239},
	pages={680-688},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2012.11.146}
}
@misc{sah08unc,
	author = 	{B. Saha et al.},
	year = 	 {2008},
	title = 	 {Uncertainty Management for Diagnostics and Prognostics of Batteries using Bayesian Techniques},
	pages = 	 {1-8},
	isbn = 	 {1095-323X}
}
@article{zha20ide,
	author={Y. Zhang et al.},
	year={2020},
	title={Identifying degradation patterns of lithium ion batteries from impedance spectroscopy using machine learning.},
	journal={Nature Communications},
	volume={11},
	number={1},
	pages={1706},
	isbn={2041-1723},
	doi={10.1038/s41467-020-15235-7}
}
@article{ric17gau,
	author={R. Richardson et al},
	year={2017},
	title={Gaussian process regression for forecasting battery state of health},
	journal={arXiv.org},
	volume={357},
	number={C},
	isbn={2331-8422},
	doi={10.1016/j.jpowsour.2017.05.004}
}
@article{koz03ele,
	author={J. Kozlowski},
	year={2003},
	title={Electrochemical cell prognostics using online impedance measurements and model-based data fusion techniques},
	volume={7},
	pages={3257-3270},
	isbn={1095-323X}
}
@article{han18NN,
	author={M. Hannan et al.},
	year={2018},
	title={Neural Network Approach for Estimating State of Charge of Lithium-Ion Battery Using Backtracking Search Algorithm},
	journal={IEEE Access},
	volume={6},
	pages={10069},
	isbn={2169-3536},
	doi={10.1109/ACCESS.2018.2797976}
}
@misc{A123_14bat,
	author = 	 {anonymous},
	year = 	 {2014},
	title = 	 {Battery Pack Design, Validation,and Assembly Guide using A123 Systems AMP20M1HD-A Nanophosphate®Cells},
	journal = 	 {User guide},
	url = 	 {https://formula-hybrid.org/wp-content/uploads/A123_AMP20_battery_Design_guide.pdf}
}
@article{ber16onl,
	author={M. Berecibara et al.},
	year={2016},
	title={Online state of health estimation on NMC cells based on predictive analytics},
	journal={Journal of Power Sources},
	volume={320},
	pages={239-250},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2016.04.109}
}
@article{li18aqu,
	author={Y. Li et al.},
	year={2018},
	title={A quick on-line state of health estimation method for Li-ion battery with incremental capacity curves processed by Gaussian filter},
	journal={Journal of Power Sources},
	volume={373},
	pages={40-53},
	isbn={0378-7753},
	doi={10.1016/j.jpowsour.2017.10.092}
}
@article{jal15cyc,
	author={K. Jalkanen et al.},
	year={2015},
	title={Cycle aging of commercial NMC/graphite pouch cells at different temperatures},
	journal={Applied Energy},
	volume={154},
	number={C},
	pages={160-172},
	isbn={0306-2619},
	doi={10.1016/j.apenergy.2015.04.110}
}
@inproceedings{huo20dyn,
	author={M. Huotari, \textit{et al.}},
	year={forthcoming},
	month={November 13-17, 2020},
	title={A Dynamic Battery State-of-Health Forecasting Model for Electric Trucks: Li-Ion Batteries Case Study},
	publisher={ASME},
	address={USA},
	doi={https://dx.doi.org/10.10.1115/IMECE2020-22453}
}


